Mechanical State Estimation with a Polynomial-Chaos-Based Statistical Finite Element Method

The Statistical Finite Element Method (statFEM) offers a Bayesian framework for integrating computational models with observational data, thus providing improved predictions for structural health monitoring and digital twinning. This paper presents an efficient sampling-free statFEM tailored for non-conjugate, non-Gaussian prior probability densities. We assume that constitutive parameters, modeled as weakly stationary random fields, are the primary source of uncertainty and approximate them using Karhunen-Lo\`eve (KL) expansion. The resulting stochastic solution field, i.e., the displacement field, is a non-stationary, non-Gaussian random field, which we approximate via Polynomial Chaos (PC) expansion. The PC coefficients are determined through projection using Smolyak sparse grids. Additionally, we model the measurement noise as a stationary Gaussian random field and the model misspecification as a mean-free, non-stationary Gaussian random field, which is also approximated using KL expansion. The coefficients of the KL expansion are treated as hyperparameters. The PC coefficients of the stochastic posterior displacement field are computed using the Gauss-Markov-K\'alm\'an filter, while the hyperparameters are determined by maximizing the marginal likelihood. We demonstrate the efficiency and convergence of the proposed method through one- and two-dimensional elastostatic problems.

==> packages/commands.tex <==
% All the unified commands to formulate the response are defined here. These commands make a unified response template. 
% Forked: Vahab Narouie, Teschnische Universität Braunschweig, 2023
% requires packages:
% To check whether the document is in its final version or not
\RequirePackage{ifdraft}
% To color text
\RequirePackage{xcolor}
% To make smart references
\RequirePackage{cleveref}
%
\geometry{
  a4paper,
  % width=597.50787pt,
  left=15mm,
  right=15mm,
  top=15mm,
  bottom=25mm,
  marginparwidth=15mm
}
%
\renewcommand\Affilfont{\itshape\small}

% Counter for comments
\newcounter{commentcnt}
% Refine the comment counters by using the Arabic numbering system. Notice that the new counter {commentcnt} automatically creates \thecommentcnt as a new command, which has to be overwritten.
\renewcommand{\thecommentcnt}{\arabic{commentcnt}}
% To use cleveref with this environment
\Crefname{commentcnt}{Comment}{Comment}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% Environments for comments and replies
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newenvironment{ReviewerComment}{\noindent\begin{minipage}[t]{\textwidth}\noindent \textbf{Comment \refstepcounter{commentcnt}{\thecommentcnt}:} \begin{quotation}
      \noindent
      \begin{em}}
        {\end{em}
    \end{quotation}\vspace{1ex}\end{minipage}}
%
\newenvironment{ReviewerCommentReprise}{\noindent\vspace{-1.25cm}%
  \begin{quotation}\noindent\begin{em}}{\end{em}\end{quotation}}
%
\newenvironment{ReviewerReply}{\noindent \textbf{Feedback: } \begin{quotation}\begin{em}}{\end{em}\end{quotation}}
%
\newenvironment{GuestEditorComment}{\noindent\begin{minipage}[t]{\textwidth}\noindent \textbf{Comment \refstepcounter{commentcnt}{\thecommentcnt} (Guest Editor): } \begin{quotation}\noindent\begin{em}}{\end{em}\end{quotation}\vspace{1ex}\end{minipage}}
%
\newenvironment{AssociateEditorComment}{\noindent\begin{minipage}[t]{\textwidth}\noindent \textbf{Comment \refstepcounter{commentcnt}{\thecommentcnt} (Associate Editor): } \begin{quotation}\noindent\begin{em}}{\end{em}\end{quotation}\vspace{1ex}\end{minipage}}
%
\newenvironment{AreaEditorComment}{\noindent\begin{minipage}[t]{\textwidth}\noindent \textbf{Comment \refstepcounter{commentcnt}{\thecommentcnt} (Area Editor): }\nopagebreak \begin{quotation}\noindent\begin{em}}{\end{em}\end{quotation}\vspace{1ex}\end{minipage}}
%
\newenvironment{EditorComment}{\noindent\begin{minipage}[t]{\textwidth}\noindent \textbf{Comment \refstepcounter{commentcnt}{\thecommentcnt} (Editor): } \begin{quotation}\noindent\begin{em}}{\end{em}\end{quotation}\vspace{1ex}\end{minipage}}
%
\newenvironment{EditorInChiefComment}{\noindent\begin{minipage}[t]{\textwidth}\noindent \textbf{Comment \refstepcounter{commentcnt}{\thecommentcnt} (Editor in Chief): } \begin{quotation}\noindent\begin{em}}{\end{em}\end{quotation}\vspace{1ex}\end{minipage}}
%
\newenvironment{MetaReviewComment}{\noindent\begin{minipage}[t]{\textwidth}\noindent \textbf{Comment \refstepcounter{commentcnt}{\thecommentcnt} (Meta-review): } \begin{quotation}\noindent\begin{em}}{\end{em}\end{quotation}\vspace{1ex}\end{minipage}}
%
\newenvironment{Answer}{\noindent \textbf{Response: }\color{blue}}{\\[.3cm]}
%
\newenvironment{AnswerInBetween}{\noindent \textbf{Response: }}{\vspace{.3cm}}
%
% \newcommand{\NoteInEvidence}[1]{\color{GreenYellow}{\textbf{#1}}}


\newcommand{\NoteInEvidence}[1]{\ifoptiondraft{\hl{#1}}{}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% Task difficulty assessment and work status boxes
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\TaskEstimationBox}[2]{%
  \ifoptiondraft{\newline \parbox{1.0\linewidth}{\hfill \hfill {\colorbox{#2}{\color{White} \textbf{#1}}}}}%
  {}%
}
%
\def\WorkInProgressRevTask {\TaskEstimationBox{Work in progress}{Cyan}}
\def\AlmostDoneRevTask {\TaskEstimationBox{Almost there}{NavyBlue}}
\def\RevTaskDone {\TaskEstimationBox{Done}{Blue}}
%
\def\NotEstimatedRevTask {\TaskEstimationBox{Effort not estimated}{Gray}}
\def\EasyRevTask {\TaskEstimationBox{Feasible}{ForestGreen}}
\def\MediumRevTask {\TaskEstimationBox{Medium effort}{Orange}}
\def\TimeConsumingRevTask {\TaskEstimationBox{Time-consuming}{Bittersweet}}
\def\HardRevTask {\TaskEstimationBox{Hard one}{Sepia}}
\def\DeathRevTask {\TaskEstimationBox{Death}{Black}}
%
\newcommand{\Assignment}[1]{
  %
  \ifoptiondraft{%
    \newline \parbox{1.0\linewidth}{\hfill \hfill \color{black}\textbf{Assignment:} #1}%
  }{}%
}

%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Put some space to separate reviewers' comments
%
\newcommand{\SkipSpaceForReviewerComments}{\vspace{6em}}

%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Add notes to be removed when the letter is not a draft anymore
%
% To color text
\RequirePackage{xcolor}
\newenvironment{NoteForAuthors}%
{\ifoptiondraft{%
    \noindent%
    \colorbox{gray}%
    {\color{white} Note: }%
    \color{orange}%
    \begin{em}%
      }{}%
      }%
      {\ifoptiondraft{%
      \normalcolor%
    \end{em}%
  }{}%
}

%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Highlight changes in revised manuscripts
%
% To color text
\RequirePackage{xcolor}
% To create side-notes
\RequirePackage{marginnote}
% Change the following line for larger (or narrower) side spaces
\setlength{\marginparwidth}{1cm}
% Change the following line for bigger (or smaller) fonts
\renewcommand*{\marginfont}{\footnotesize}

\newenvironment{HlRev}[1][]{%
  % No hyperrefs here
  \begin{NoHyper}
    % Change the colour to the olive green
    \color{OliveGreen}%
    % If an argument is passed, it is used as the number of the comment in a side note
    \ifx\newenvironment#1\newenvironment\else\marginnote{Comment #1}\fi%
    %
    }{%
    % Restores the normal color
    \normalcolor%
    % Restores the normal hyperref behavior
  \end{NoHyper}%
}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%


==> packages/pkgloading.tex <==
% To allow for extra UTF-8 characters in the text
\usepackage[utf8]{inputenc}
% The Helvetica font
\usepackage{helvet}
% To use colors
\usepackage[usenames,dvipsnames]{xcolor}
% To nicely format URLs
\usepackage{url}
% For using inparaenum, basically
\usepackage{paralist}
% For adding TODO notes
\usepackage[obeyDraft,textsize=tiny,backgroundcolor=blue!10]{todonotes}
% To add author blocks to the front-matter
\usepackage{authblk}
% To create linked anchors on top of references
%\usepackage[pdfborder={0 0 0}]{hyperref}
% To play around with enumerations and bullet lists
\usepackage{enumitem}
% To load hyphenation rules and other Locale-standardised things
\usepackage[english]{babel}
% For the letter-like symbol, {\Letter}
\usepackage{marvosym}
% To comment
\usepackage{comment}
% To adjust margins
\usepackage{geometry}
% Fancy HREFs
\usepackage[draft=true]{hyperref}
%\usepackage{nohyperref}
% Fancy enumerations and itemized lists
\usepackage{enumitem}
% For \mathbb command, among the others
\usepackage{amsfonts}
% For creating side-notes
\usepackage{marginnote}
% For specifying keywords and acronyms
\usepackage[nonumberlist,acronym,sanitize=none]{glossaries}
\glsdisablehyper
% For equations, arrays of equations, defining operator names, etc.
\usepackage{amsmath}
% For cursive math
\usepackage{mathrsfs}
% For math symbols, such as \nexists
\usepackage{amssymb}
% To check whether the document is in its final version or not
\usepackage{ifdraft}
% To highlight text
\usepackage{soul}
% For decent formatting of numbers (and a wonderful system for numeric columns in tables, ``S'')
\usepackage{siunitx}
% To create right arrows in text environment
\usepackage{textcomp}
% For smart references
\usepackage[capitalise,nameinlink]{cleveref}
\crefname{algocf}{algorithm}{algorithms}
\Crefname{algocf}{Algorithm}{Algorithms}
% To cross-reference other documents
\usepackage{xr}
% To produce hypertext links in the document
\usepackage{hyperref}
% Bibliography management
\usepackage[square,comma,numbers,sort,sectionbib,nonamebreak]{natbib}
